BERTnesia: Investigating the capture and forgetting of knowledge in BERT

Probing complex language models has recently revealed several insights into linguistic and semantic patterns found in the learned representations. In this paper, we probe BERT specifically to understand and measure the relational knowledge it captures. We utilize knowledge base completion tasks to probe every layer of pre-trained as well as fine-tuned BERT (ranking, question answering, NER). Our findings show that knowledge is not just contained in BERT's final layers. Intermediate layers contribute a significant amount (17-60%) to the total knowledge found. Probing intermediate layers also reveals how different types of knowledge emerge at varying rates. When BERT is fine-tuned, relational knowledge is forgotten but the extent of forgetting is impacted by the fine-tuning objective but not the size of the dataset. We found that ranking models forget the least and retain more knowledge in their final layer. We release our code on github to repeat the experiments.

==> evolution.tex <==
% \section{Experimental Results}

% \todo{I would rather  state the RQs in the intro and refer to them.}

% In this section, we seek to answer the following research questions with the methodology just outlined.


% \begin{itemize}
%     \item How much knowledge is stored in the intermediary layers of BERT? Does knowledge grow at equal rates for all relationship types?
%     \item
    
% \end{itemize}

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{plots/old/default/multiple-means/multiple-means-P-AT-1.png}
    \caption{Mean P@1 performance of the default model on different probing datasets.}
    \label{fig:bert_layers}
\end{figure}

%  Default trex parallel
\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{plots/old/default/parallel/TREx-P-AT-1.png}
    \caption{Default models P@1 performance on the 41 T-REx relations over the layers}
    \label{fig:trex_all_default}
\end{figure}



%  Default sqaud ranking ner on 2 datasets
\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{plots/old/default-squad2-qa-ner-msmarco-ranking/means/TREx-means-P-AT-1.png}
    \caption{Mean performance on T-REx for Default, QA SQuAD 2, Ranking on MSMARCO, NER on Conll-2003}
    \label{fig:layerwise_mixed}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{plots/old/default-squad2-qa-ner-msmarco-ranking/means/ConceptNet-test-P-AT-1.png}
    \caption{Mean performance on ConceptNet for Default, QA SQuAD 2, Ranking on MSMARCO, NER on Conll-2003}
    \label{fig:my_label}
\end{figure}


% Default and all squad models means on trex
\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{plots/old/default-and_all_squad_models/means/TREx-means-P-AT-1.png}
    \caption{Mean performance on T-REx for Default, QA SQuAD 1.1, QA SQuAD 2, MLM SQuAD 2}
    \label{fig:trex_squad}
\end{figure}

% Comparing training objective on SQuAD:
% Default, QA Squad2 and mlm squad
\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{plots/old/compare-objective-squad/means/TREx-means-P-AT-1.png}
    \caption{Comparing the different training objectives on SQuAD 2: MLM, QA and the default model for comparion. Shown is the precision at 1 on the T-REx probe}
    \label{fig:my_label}
\end{figure}

% Comparing all mlm model
% Default, mlm squad, mlm msmarco
\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{plots/old/compare_datasets_mlm_models/means/ConceptNet-test-P-AT-1.png}
    \caption{Comparing MLM models on different datasets: We show MLM on SQuAD 2, MSmarco and the default model which has been trained on MLM during pre-training. Shown is the precision at 1 on the ConceptNet probe}
    \label{fig:conceptnet_mlm}
\end{figure}
    


\section{Evolution analysis of knowledge capture in BERT}

Previous work has shown that BERT is capable of remembering factual knowledge. The LAMA probe task enabled researchers to quantify the ability of BERT to answer factual knowledge questions. 

In our experiments, we probe BERT not just at the last layer to estimate the extent of knowledge capture but also all the intermediary layers to observe the evolution of knowledge capture. Figure~\ref{fig:bert_layers} shows the performance of each layer on the LAMA probe tasks for Default-BERT. In the case of Default-BERT, the task that the model was trained on is the same as that of the probe (MLM), however, the training data distributions are different. From the figure we see that the amount of knowledge captured increases steadily with each additional layer. This implies that the embedding space learned at each layer gets progressively better oriented for identifying factual knowledge. In other words, BERT remembers more factual knowledge in its last layer than its previous layers. This is distinctly different from previous studies on linguistic pattern probing where results indicate that such patterns are best captured in the intermediary layers. Hence BERT can capture structure early on but specific factual knowledge emerges best at the end.



These trends are from an aggregate of all relationship types. When observing single relationship types however, the plot literally and figuratively thickens. We see that not all relationship types are best captured in the last layer. To quantify this observation we compute a simple win/loss ratio defined as follows:





From table~\ref{tab:win_loss}, we see that for 25\% of relations, BERT essentially forgets at the last layer. When probing for knowledge just measuring the probe performance on the last layer may be misleading. Essentially the embeddings for certain relational knowledge is better captured at the lower layers. 

\begin{itemize}
    \item more detail on what bert default forgets
    \item should we talk about the win loss for other models here
\end{itemize}

Figure~\ref{fig:trex_all_default} shows the amount of knowledge captured at each layer for the TReX probe. Another surprising finding here is the acceleration rate of various relations. Certain relations are easier to capture early on whereas others drastically improve layer 9 onwards. 

\begin{itemize}
    \item show examples of relations that are different. Jonas needs to give me the nams of relationships.
\end{itemize}


%In the following table we show the top 3 and bottom 3 relations per layer according to LAMA. 

%Another observation here is the variation in the rate of knowledge capture. Certain relations like x,y,z grow rapidly layer 8 onwards whereas other relations grow more gradually. 
A small proportion of relations also seem to be forgotten as the knowledge captured is highest in the intermediary layer. The reason why forgetting happens can be attributed to several factors but in this paper we limit ourselves to investigating the impact of the training data used to fine tune the decoding head. More specifically, our hypothesis is -- does the the relation distribution of the fine tuning data impact knowledge capture of certain relations?

To answer this question, we first estimate the frequency of each relation from the Google TReX dataset in the fine tuning data. We constructed regular expressions for each relation type and counted the matched sentences in the fine tuning data. Table Y shows the relative proportion of each relation.

\textit{Pie chart of relations. ToDo. If we have time}.

From here we see that certain relations are better represented in the training data which leads to better overall performance in the intermediary layers generally. However we see that for certain relations such as x, even a small amount of training data can help the model easily capture this knowledge. This indicates that in the embedding space, certain relations are much easier to separate even with a small amount of fine tuning data. These relations are likely to have more distinct semantic meaning like x rather than y. 

In the next section we investigate knowledge capture when BERT is fine tuned on a downstream task. 


==> intro.tex <==
\section{Introduction}

\todo{Shorten general intro}
Large pre-trained language models like \bert{}~\cite{devlin2018bert} have heralded an \textit{Imagenet} moment for NLP with not only significant improvements made to traditional tasks such as question answering and machine translation but also in the new areas such as knowledge base completion. \bert{} has over 100 million parameters and essentially trades off transparency and interpretability for performance.
\textbf{Why is Probing as a technique is useful..why is it a good way to measure knowledge stored.}
To better understand the inner workings of \bert{} and other complex language models, probing is a commonly used technique. Probing in general is a procedure by which one tests for a specific pattern by constructing inputs whose expected output would not be possible to predict without said pattern. While a large body of work exists on probing \bert{} for linguistic patterns and semantics, little work exists on probing these models for the knowledge they store.

%without any fixed schema.
%, flexible querying with no restrictions on relationship types, easy to extend with fine tuning and are self-supervised

\citet{petroni2019language} probed \bert{} and other language models for relational knowledge (e.g. \textit{Trump} is the president of the \textit{USA}) in order to determine the potential of using language models as automatic knowledge bases. They inherently measured the amount of knowledge stored in \bert{} by designing a cloze statement probe task akin to knowledge base completion tasks ([MASK] is the president of the \textit{USA} -- predict the masked word). Since \bert{} is pre-trained used masked language modeling (MLM), they were able to estimate the amount of knowledge contained by measuring the performance of the MLM decoding head for their cloze tasks.


%Such cloze statements are usually extracted from sources like Wikipedia or created from templates specific to each relationship type. We describe these probe tasks in detail in Section~\ref{sec:probes} and denote them henceforth as knowledge probes. 
While researchers have been able to measure and characterize knowledge stored in \bert{} using such probe tasks, we are still in the dark regarding \emph{how} this knowledge is stored in \bert{} and \emph{how} this knowledge is affected when \bert{} is fine tuned. 

\textbf{Our Contribution} In this paper we study the emergence of knowledge through the layers in \bert{} by devising a knowledge probing procedure to estimate knowledge contained in every layer and not just the last (as in~\cite{petroni2019language}). While this type of layer-by-layer probing has been conducted for syntactic, grammatical and semantic patterns; knowledge probing has only been conducted on final layer representations. Observing only the final layer (as we will show in our experiments)  (i)  underestimates the amount of knowledge (ii) does not reveal how knowledge emerges. 

Furthermore we explore how knowledge is impacted when fine-tuning on knowledge intensive tasks such as question answering and ranking. More specifically, we seek to empirically answer the following research questions: 

%A  In this paper we utilize knowledge probes to further investigate layer-by-layer the ability of BERT, both pre-trained and fine tuned, to capture and manifest various forms of relational knowledge. 

%we first trained decoding MLM heads for each layer. Then we measured the knowledge captured at each layer with knowledge probes spanning several relationship types and domains. We conducted these measurements for a pretrained BERT model, BERT fine tuned for reading comprehension, BERT fine tuned for QA and BERT fine tuned for passage ranking. Finally we compared, contrasted and characterized the evolution of knowledge in order to answer the following research questions:


%The key idea is to measure the ability of each layer's embeddings to detect a specific pattern in a supervised manner. By identifying which patterns emerge and when they do, we can start to understand the underpinnings of BERT and reason to the effectiveness of it in a multitude of tasks.





%\todo{questions are still vague cause i dont have many details in the intro}
\begin{itemize}
    \item Is probing the last layer sufficient in estimating the knowledge contained in BERT? Do intermediary layers capture knowledge not present in the last layer? (Section~\ref{sec:intermediate})
    \item Does fine tuning BERT lead to prior knowledge being forgotten or does fine tuning improve knowledge capture? (Section~\ref{sec:intermediate})
    \item Does all knowledge emerge at the same rate? Do certain types of relational knowledge emerge more rapidly? (Section~\ref{sec:evolution})
    \item To what extent is forgetting influenced by volume and veracity of the fine tuning dataset? (Section~\ref{sec:data_size})
    \item To what extent is forgetting influenced by the fine tuning objective? (Section~\ref{sec:finetuning})
   
\end{itemize}


Our findings indicate that for pretrained \bert{} (i) a significant amount of knowledge is stored in the intermediate layers ($\~24\%$ on average) (ii) not all relation knowledge are captured gradually through the layers however with x\% essentially doubling in the last layer and 7\% of relationship types being maximal in an intermediate layer. 
. For fine tuned \bert{}, knowledge captured is not always maximal in the final layers due to learning task specific patterns. 43\% of relationship types are better captured in intermediate layers for a question answering model (named \qasquad{} in our experiments). We found that (i) the dataset size plays a major role when the training objective is fixed -- smaller datasets make \bert{} easily forget relational knowledge (ii) when the size of the dataset is fixed and training objective varies, we find that the ranking model (\rankmarco{} in our experiments) captures the most amount of knowledge hinting that ranking in comparison is a more knowledge heavy task. 

%\todo{This is a very mellow statement. A conclusion should be precise and strong.}
%When fine tuning BERT, \textbf{knowledge captured is maximal in the penultimate layers with the final layer catering more towards task specific pattern detection. }

%For fine tuned models we found that \textbf{the dataset size plays a major role when the training objective is fixed -- smaller datasets make BERT easily forget relational knowledge.} 
%\todo{Larger datasets leads to }
%When the size of the dataset is fixed and training objective varies, we find that \textbf{the ranking model captures the most amount of knowledge} hinting that ranking in comparison is a more knowledge heavy task. 


The remainder of this paper is dedicated first to situating our work in the NLP probing literature. Then we detail knowledge probes and describe our experimental settings. Finally we present evidence to substantiate the aforementioned claims. 

%Given that  here isthe complex nature of powerful models such as BERT, several studies have been proposed to probe and understand the information contained within~\cite{}. Recently, researchers have begun investigating the applicability of 

% for forgetting we should measure the amount of existing relations where precision drops and for gain in knowledge we should look at relations that were wrong before
